ANNEXE: Unified Analyzing, Answering, and Pixel Grounding for Egocentric Interaction

Egocentric interaction perception is one of the essential branches in investigating human-environment interaction, which lays the basis for developing next-generation intelligent systems. However, existing egocentric interaction understanding methods cannot yield coherent textual and pixel-level responses simultaneously according to user queries, which lacks flexibility for varying downstream application requirements. To comprehend egocentric interactions exhaustively, this paper presents a novel task named Egocentric Interaction Reasoning and pixel Grounding (Ego-IRG). Taking an egocentric image with the query as input, Ego-IRG is the first task that aims to resolve the interactions through three crucial steps: analyzing, answering, and pixel grounding, which results in fluent textual and fine-grained pixel-level responses. Another challenge is that existing datasets cannot meet the conditions for the Ego-IRG task. To address this limitation, this paper creates the Ego-IRGBench dataset based on extensive manual efforts, which includes over 20k egocentric images with 1.6 million queries and corresponding multimodal responses about interactions. Moreover, we design a unified ANNEXE model to generate text- and pixel-level outputs utilizing multimodal large language models, which enables a comprehensive interpretation of egocentric interactions. The experiments on the Ego-IRGBench exhibit the effectiveness of our ANNEXE model compared with other works.

==> sec/3_finalcopy.tex <==
\section{Methods}
\label{methods}
This paper investigates the problem of pixel-level grounding and with text answers in egocentric images, i.e., the simultaneous text and image responses for user prompts. 
We begin this section by formally describing the task Ego-IPCG in Sec. \ref{sec::method-taskD}. And In Sec. \ref{sec::method-OverA} we introduce our model DCGNet, which can understand the context of the input text prompts and egocentric images

\subsection{Task Definition}
\label{sec::method-taskD}
xxx

\subsection{Overall Architecture}
\label{sec::method-OverA}
xxx

\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_method.tex <==
\section{Methods}
\label{methods}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{fig_2}
	\caption{Overall architecture of the proposed ANNEXE model.}
	\label{fig:2}
\end{figure*}


This paper introduces a novel task called Ego-IRG, which aims to generate both the text- and pixel-level responses to the user query about the interaction depicted in the egocentric image. 
We begin this section by formally describing the task Ego-IRG in Sec. \ref{sec::method-taskD}. 
In Sec. \ref{sec::method-OverA}, we introduce our model ANNEXE and its sub-modules in detail. 
Finally, the description of the proposed Ego-Inter dataset is described in Sec. \ref{sec::method-dataset}.

\subsection{Task Definition}
\label{sec::method-taskD}
This paper proposes a novel task, Ego-IRG, which enables unified analysis, answering, and pixel grounding regarding interactions in egocentric images based on user queries.
Taking an egocentric image $\textbf{I}$ and a query $\textbf{T}$ as input, the primary goal of the Ego-IRG task is to analyze the interaction in $\textbf{I}$ and produce the interaction description $\textbf{R}_{D}$.
Subsequently, the Ego-IRG task involves generating the answers $\textbf{R}_{A}$ in response to the query $\textbf{T}$, along with the pixel-level mask grounding results $\textbf{R}_{M}$ of the object participating in the interaction specified in the query. 


\subsection{ANNEXE Architecture}
\label{sec::method-OverA}
To address the proposed Ego-IRG task, this paper establishes the ANNEXE model, which is the first model that can generate text-level and fine-grained pixel-level responses simultaneously for egocentric interaction understanding.
Taking an egocentric image $\textbf{I}$ and a query $\textbf{T}$ as input, the ANNEXE can achieve analysis, answering, and pixel-grounding regarding the interactions in the image.
The ANNEXE model can be divided into two parts: the reasoning module and the grounding module, as depicted in Fig. \ref{fig:2}.  
The former module is used to generate the text responses for the query, including interaction analysis (description) and answers. The latter module is designed to generate the pixel-level grounding results.
The following two sections will describe these two modules in detail.

\subsubsection{Reasoning Module}
As illustrated in Fig. \ref{fig:2}, the reasoning module mainly focuses on the text response generation regarding the query and the interaction in the image.
Due to the significant success of the MLLM, we utilize its strong capabilities of understanding and aligning the context of language and image.
Therefore, we employ a frozen prompt encoder and an image encoder to extract the representative features of the text prompt $\textbf{T}$ and input egocentric image $\textbf{I}$.
Furthermore, since the text prompt required by description and answer is different, we add an additional fixed instruction $\textbf{T}_a$ to guide MLLM to predict interaction analysis $\textbf{R}_D$.
The process of extracting the features can be represented as follows:
\begin{align}
  \textbf{F}_{enc}^{img} &= \mathcal{F}_{enc}^i(\textbf{I},W_{enc}^i), \\
  \textbf{F}_{enc}^{ins}, \textbf{F}_{enc}^{que} &= \mathcal{F}_{enc}^p(\textbf{T}_a,\textbf{T},W_{enc}^p),
  \label{eq:extract}
\end{align}
where the $\textbf{F}_{enc}^{img}$, $\textbf{F}_{enc}^{ins}$, and $\textbf{F}_{enc}^{que}$ are the extracted features of egocentric image, analysis instruction, and input query, respectively.
And the functions $\mathcal{F}_{enc}^i(\cdot)$ and $\mathcal{F}_{enc}^p(\cdot)$ represent the image encoder with the parameters of $W_{enc}^i$ and prompt encoder with the parameter of $W_{enc}^p$ respectively.

After feature extraction, the multi-modal LLM $\mathcal{F}$ is utilized to obtain two types of textual output, \emph{i.e.}, interaction analysis and answers for query.
This process can be represented as:
\begin{equation}
	\textbf{R}_{D}, \textbf{R}_{A} = \mathcal{F}(\textbf{F}_{enc}^{img}, \textbf{F}_{enc}^{ins}, \textbf{F}_{enc}^{que},W),
\end{equation}
where the $\mathcal{F}(\cdot)$ means the multi-modal LLM with the parameter of $W$.
In practice, the MLLM we used was Mini-GPT4v2, and the image and prompt encoders are frozen while the $\mathcal{F}$ is trainable.
Through this reasoning module, the MLLM can be trained to generate coherent and precise interaction descriptions and answers depending on different queries and instructions, which further enhances the capability of the model to understand the information of input texts and images.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{fig_3}
	\caption{The illustration of the proposed Ego-Inter dataset, which includes (a)(i) the egocentric image, (a)(ii) depth map, and interaction description. In addition, for each egocentric, multiple query-response-mask pairs are provided to comprehensively understand the interactions, including the single-, multi-, and no-target samples as shown in (b), (c), and (d), respectively.}
	\label{fig:3}
\end{figure*}

\subsubsection{Grounding Module}
The grounding module is incorporated to obtain the fine-grained pixel-level grounding results based on the extracted query and image features, as shown in Fig. \ref{fig:2}.
In addition, we argue that depth information is essential for understanding egocentric interactions. This is because we observed that when people perform an activity, the operating objects and hands are usually positioned in the foreground, which has a relatively clear distinction from background in depth, especially when multiple similar objects are in the scenario.
Therefore, the depth estimation branch is also integrated to help mask generation in the grounding module.

Taking the image feature $\textbf{F}_{enc}^{img}$ and the query feature $\textbf{F}_{enc}^{que}$ as the input, we first use a trainable classification index head to predict mask index, which indicates whether the targeted objects are in the image.
In this binary classification setting, if the predicted mask index is true, the pixel-level grounding mask will be generated further, while the mask prediction will not be considered if the mask index is false.
Specifically, we select some representative features $\textbf{F}_{sel}^{que}$ from the query feature $\textbf{F}_{enc}^{que}$ along with $\textbf{F}_{enc}^{img}$ as inputs to the classification index head.
In practice, the index head includes several stacked convolution-relu-pooling layers with multi-layer perceptron.
The classification process is:
\begin{equation}
	\textbf{R}_c = \mathcal{F}_c(\textbf{F}_{img},\textbf{F}_{sel}^{que}, W_c),
\end{equation}
where the $\textbf{R}_c$ is the predicted mask index result with a value of 0 or 1. 
The $\mathcal{F}_{c}(\cdot)$ means the classification index head with the parameters of $W_c$.

Furthermore, we regard depth estimation as an auxiliary task that helps the network extract features with depth characteristics.
Specifically, we add an additional depth estimation branch in the grounding module, in which a trainable ground image encoder $\mathcal{F}_{enc}^g$ is used to extract depth-aware image features $\textbf{F}_g^{img}$.
A trainable depth estimation decoder $\mathcal{F}_d$ with the parameters of $W_d$ is also utilized to predict the depth information, which will promote the encoder to learn the depth characteristics:
\begin{equation}
	\textbf{R}_d = \mathcal{F}_d(\textbf{F}_g^{img},W_d).
\end{equation}


Consequently, based on the predicted mask index $\textbf{R}_c$, extracted image feature $\textbf{F}_g^{img}$, and selected query features $\textbf{F}_{sel}^{que}$, the pixel-grounding mask prediction will be generated through the trainable depth estimation decoder.
We select the mask decoder in the Segment Anything Model (SAM) as the depth estimation decoder $\mathcal{F}_p$:
\begin{equation}
	\textbf{R}_M = \mathcal{F}_p(\textbf{F}_{g}^{img},\textbf{F}_{sel}^{que},W_p \; | \; \textbf{R}_c),
\end{equation}
where the $\textbf{R}_M$ is the generated mask, and the $W_p$ is the trainable parameter of the mask decoder.
By incorporating the grounding module, the proposed ANNEXE model can predict precise and query-orientated pixel-level masks about the egocentric interaction.



\subsubsection{Training Loss}
The training loss of the ANNEXE model consists of five parts, \emph{i.e.}, the description loss $\mathcal{L}_d$, the answer loss $\mathcal{L}_a$, the classification loss $\mathcal{L}_c$ for mask index, the depth estimation loss $\mathcal{L}_{dep}$, and the pixel grounding loss $\mathcal{L}_p$.
We use the cross entropy loss for $\mathcal{L}_d$, $\mathcal{L}_a$, and $\mathcal{L}_p$.
The binary cross entropy loss is used for $\mathcal{L}_c$, and smooth L1 loss is utilized for $\mathcal{L}_{dep}$.
Therefore, the overall loss function for the ANNEXE is:
\begin{align}
	\mathcal{L} &= \lambda_{des} \mathcal{L}_{des} + \lambda_{ans} \mathcal{L}_{ans} \\
	& + \lambda_{cls} \mathcal{L}_{cls}+	 \lambda_{dep} \mathcal{L}_{dep} + \lambda_{pxl} \mathcal{L}_{pxl},
\end{align}
where the $\mathcal{L}$ is the final loss, and the $\alpha ,\gamma ,\beta, \lambda$ are the weight of the corresponding loss function.

\begin{table}[]
\resizebox{\linewidth}{!}{
	\begin{tabular}{@{}lcccccc@{}}
		\hline
\multirow{2}{*}{Dataset} & 
\multirow{2}{*}{Ego / Exo} & \multirow{2}{*}{Interaction} & \multirow{2}{*}{Query} & \multicolumn{3}{c}{Responses} \\ \cline{5-7} 
&   &   &  & Ana. & Ans. & Msk \\ \hline
SAM-1B & Exo &N &N & N &N  &Y \\ \hline
GranD & Exo & N & N & Y & N & Y \\ \hline
RefCOCO &Exo &N &Y &N &N &Y \\ \hline
RefCOCO+&Exo &N &Y &N &N &Y \\ \hline
RefClef&Exo &N &Y &N &N &Y \\ \hline
G-Ref&Exo &N &Y &N &N &Y \\ \hline
VISOR & Ego & Y & Y & N & Y & Y \\ \hline
EPIC-KITCHENS & Ego & Y & N & - & - &\\ \hline
EGTEA & Ego & Y & N & - & - & \\ \hline
HOI4D & Ego & Y & N & N & Y & \\ \hline
Ego4D &Ego &Y &Y &N &N & \\ \hline
EgoHOS & Ego & Y & N & N & Y & \\ \hline
VISOR-NVOS & Ego & Y & N & N & Y &\\ \hline
Ego-Inter & Ego  & Y  & Y & Y & Y   &  \\ \hline
	\end{tabular}}
\caption{Ego-Inter versus other datasets. Obviously, Ego-Inter is the first dataset that provides unified query-answer, analysis, and pixel-level grounding results for egocentric understanding. The Ana. means analysis description for interactions, the Ans. means the answer for query, and the Msk means the pixel grounding mask.}
\label{tab:1}
\end{table}



\subsection{Ego-Inter Dataset}
\label{sec::method-dataset}
To establish a comprehensive system for understanding egocentric interactions, we create a novel task, Ego-IRG.
The objective of the Ego-IRG task is to generate the \textit{interaction descriptions, answers, and pixel-level grounding responses} simultaneously based on the input text queries and egocentric images.
To encourage future study of the Ego-IRG task, we present a high-quality dataset Ego-Inter with extensive labor.
This dataset is built upon the HOI4D dataset, and we use a stage-wise annotation pipeline that consumes extensive manual efforts to re-label the dataset with queries and corresponding text- and pixel-level responses.
Different with other related datasets, the Ego-Inter dataset is the first that provides the textual responses and pixel-level grounding masks for egocentric interaction understanding. The comparison of Ego-Inter dataset with others is shown in Tab. \ref{tab:1}. 


\textbf{Structure and Scale.} 
The Ego-Inter dataset comprises over 1.6 million queries and corresponding text- and pixel-level response pairs constructed on 20,681 RGB-D egocentric images.
Specifically, each image corresponds to multiple queries, with each query providing the textual response and fine-grained pixel-level grounding mask.
The textual responses include two types of languages, i.e., the description of the interaction in the image and the answers to the query.
Furthermore, the query is not limited to single-target involving interactions. Multi-target and no-target queries are also provided in the Ego-Inter dataset, which shows the diversity of the dataset, as shown in Fig. \ref{fig:3}. 
More explanations for the dataset can be referred in Appendix A.1.

\textbf{Step-wise Annotation Pipeline.}
To efficiently build up the dataset that meets the requirements of the Ego-IRG task, we implemented a semi-automated annotation pipeline from coarse to fine. 
Specifically, the annotation pipeline includes three steps: interaction classification, hand-object mask generation, and query-response generation.
In the first step, interaction classification, the experts are employed to classify the aligned RGB-D images to determine whether interactions are occurring. As a result, the images are divided into two categories: with and w/o interactions. For samples that include interactions, the description of the interaction is generated manually.
In the second step, masks for the hands and interacting objects are generated semi-automatically (as detailed in Appendix A.2).
Finally, queries and textual responses are created manually, while the corresponding pixel-level grounding masks are generated automatically.


\textbf{Evaluation Criteria}: We introduce a benchmarking for Ego-IRG, \textbf{yielding a validation set of 2.5K images and xxx query-response-mask pairs, and a test set of 5K images and xx query-response-mask pairs. }
Four key aspects are evaluated: i) generated
interaction description quality, ii) quality of generated answers for queries, iii) pixel-level grounding ability.
Validation metrics include METEOR and CIDEr
for interaction descriptions and answers, mIoU for pixel-level grounding. (refer to Appendix A.3 for details).



